Setting AI in context: A case study on defining the context and operational design domain for automated driving

[Context and motivation] For automated driving systems, the operational context needs to be known in order to state guarantees on performance and safety. The operational design domain (ODD) is an abstraction of the operational context, and its definition is an integral part of the system development process. [Question / problem] There are still major uncertainties in how to clearly define and document the operational context in a diverse and distributed development environment such as the automotive industry. This case study investigates the challenges with context definitions for the development of perception functions that use machine learning for automated driving. [Principal ideas/results] Based on qualitative analysis of data from semi-structured interviews, the case study shows that there is a lack of standardisation for context definitions across the industry, ambiguities in the processes that lead to deriving the ODD, missing documentation of assumptions about the operational context, and a lack of involvement of function developers in the context definition. [Contribution] The results outline challenges experienced by an automotive supplier company when defining the operational context for systems using machine learning. Furthermore, the study collected ideas for potential solutions from the perspective of practitioners.

==> macro-editing.tex <==
\usepackage{ifthen}
\usepackage{amssymb}
\newboolean{showcomments}
\setboolean{showcomments}{true} % toggle to show or hide comments and proof reading markings


\ifthenelse{\boolean{showcomments}}
  {\newcommand{\nb}[2]{
    \fcolorbox{gray}{yellow}{\bfseries\sffamily\scriptsize#1}
    {\sf\small$\blacktriangleright$\textit{#2}$\blacktriangleleft$}
   }
   \newcommand{\version}{\emph{\scriptsize$-$working$-$}}
  }
  {\newcommand{\nb}[2]{}
   \newcommand{\version}{}
  }

\newcommand\martin[1]{\nb{Hans-Martin}{#1}}
\newcommand\eric[1]{\nb{Eric}{#1}}
\newcommand\jennifer[1]{\nb{Jennifer}{#1}}
\newcommand\padmini[1]{\nb{Padmini}{#1}}
\newcommand\olof[1]{\nb{Olof}{#1}}
\newcommand\oliver[1]{\nb{Oliver}{#1}}
\newcommand\stefan[1]{\nb{Stefan}{#1}}

% Macros for proof-reading
\usepackage[normalem]{ulem} % for \sout
\usepackage{xcolor}

\ifthenelse{\boolean{showcomments}}
  {
  \newcommand{\ra}{$\rightarrow$}
  \newcommand{\ugh}[1]{\textcolor{red}{\uwave{#1}}} % please rephrase
  \newcommand{\ins}[1]{\textcolor{blue}{\uline{#1}}} % please insert
  \newcommand{\del}[1]{\textcolor{red}{\sout{#1}}} % please delete
  \newcommand{\chg}[2]{\textcolor{red}{\sout{#1}}{\ra}\textcolor{blue}{\uline{#2}}} % please change
  \newcommand{\inspar}[1]{\color{blue}{#1}\color{blue}} % Put edit comments in a really ugly standout display
  }
  {
  \newcommand{\ra}{}
  \newcommand{\ugh}[1]{#1} % Keeps original
  \newcommand{\ins}[1]{#1} % Inserts text
  \newcommand{\del}[1]{} % Removes text
  \newcommand{\chg}[2]{#2} % Keeps only the proposed change
  \newcommand{\inspar}[1]{} % Removes edit and box
  
  }

==> nice_tables.tex <==
%% Nice Tables
\usepackage{booktabs}
\usepackage{array}
\usepackage{colortbl}
\usepackage{multirow}
\usepackage{longtable}


\newcolumntype{v}[1]{>{\raggedright \hspace {0pt}}p{#1}}
